Transforming Wikipedia into Augmented Data for Query-Focused Summarization

The limited size of existing query-focused summarization datasets renders training data-driven summarization models challenging. Meanwhile, the manual construction of a query-focused summarization corpus is costly and time-consuming. In this paper, we use Wikipedia to automatically collect a large query-focused summarization dataset (named WIKIREF) of more than 280, 000 examples, which can serve as a means of data augmentation. We also develop a BERT-based query-focused summarization model (Q-BERT) to extract sentences from the documents as summaries. To better adapt a huge model containing millions of parameters to tiny benchmarks, we identify and fine-tune only a sparse subnetwork, which corresponds to a small fraction of the whole model parameters. Experimental results on three DUC benchmarks show that the model pre-trained on WIKIREF has already achieved reasonable performance. After fine-tuning on the specific benchmark datasets, the model with data augmentation outperforms strong comparison systems. Moreover, both our proposed Q-BERT model and subnetwork fine-tuning further improve the model performance. The dataset is publicly available at https://aka.ms/wikiref.

==> name.tex <==
@inproceedings{klein-EtAl:2017:ACL-2017-System-Demonstrations,
    title = "{O}pen{NMT}: Open-Source Toolkit for Neural Machine Translation",
    author = "Klein, Guillaume  and
      Kim, Yoon  and
      Deng, Yuntian  and
      Senellart, Jean  and
      Rush, Alexander",
    booktitle = "Proceedings of {ACL} 2017, System Demonstrations",
    month = jul,
    year = "2017",
    address = "Vancouver, Canada",
    publisher = "Association for Computational Linguistics",
    pages = "67--72",
}
@inproceedings{ott2019fairseq,
    title = "fairseq: A Fast, Extensible Toolkit for Sequence Modeling",
    author = "Ott, Myle  and
      Edunov, Sergey  and
      Baevski, Alexei  and
      Fan, Angela  and
      Gross, Sam  and
      Ng, Nathan  and
      Grangier, David  and
      Auli, Michael",
    booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics (Demonstrations)",
    month = jun,
    year = "2019",
    address = "Minneapolis, Minnesota",
    publisher = "Association for Computational Linguistics",
    pages = "48--53",
}
@inproceedings{sennrich-haddow-birch:2016:P16-12,
    title = "Neural Machine Translation of Rare Words with Subword Units",
    author = "Sennrich, Rico  and
      Haddow, Barry  and
      Birch, Alexandra",
    booktitle = "Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = aug,
    year = "2016",
    address = "Berlin, Germany",
    publisher = "Association for Computational Linguistics",
    pages = "1715--1725",
}
@inproceedings{kingma2014adam,
  title = "Adam: {A} Method for Stochastic Optimization",
  author = "Diederik P. Kingma and
               Jimmy Ba",
  booktitle = "3rd International Conference on Learning Representations",
  month = may,
  year = "2015",
  address = "San Diego, CA, USA",
  pubilsher = {OpenReview.net},
}
@inproceedings{he2016deep,
  title="Deep residual learning for image recognition",
  author="He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian",
  booktitle="Proceedings of the IEEE conference on computer vision and pattern recognition",
  month=jun,
  year="2016",
  address="Las Vegas, NV, USA",
  publisher="IEEE Computer Society",
  pages="770--778",
}
@article{ba2016layer,
  title="Layer normalization",
  author="Ba, Jimmy Lei and Kiros, Jamie Ryan and Hinton, Geoffrey E",
  journal="arXiv preprint arXiv:1607.06450",
  month = jul,
  year="2016",
}
@inproceedings{cho2014learning,
    title = "Learning Phrase Representations using {RNN} Encoder{--}Decoder for Statistical Machine Translation",
    author = {Cho, Kyunghyun  and
      van Merri{\"e}nboer, Bart  and
      Gulcehre, Caglar  and
      Bahdanau, Dzmitry  and
      Bougares, Fethi  and
      Schwenk, Holger  and
      Bengio, Yoshua},
    booktitle = "Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing ({EMNLP})",
    month = oct,
    year = "2014",
    address = "Doha, Qatar",
    publisher = "Association for Computational Linguistics",
    pages = "1724--1734",
}
@article{10.5555/944919.944966,
    author = {Bengio, Yoshua and Ducharme, R\'{e}jean and Vincent, Pascal and Janvin, Christian},
    title = {A Neural Probabilistic Language Model},
    year = {2003},
    volume = {3},
    issn = {1532-4435},
    journal = {Journal of Machine Learning Research},
    month = {March},
    pages = {1137–1155},
    numpages = {19}
}
@inproceedings{mikolov2010recurrent,
  author={Mikolov, Tomas and Karafi{\'a}t, Martin and Burget, Lukas and Cernock{\`y}, Jan and Khudanpur, Sanjeev},
  title={Recurrent neural network based language model},
  booktitle={Proceedings of the Conference of the International Speech Communication Association},
  year={2010},
  address={Makuhari, Chiba, Japan},
  pages={1045--1048}
}
@inproceedings{vaswani-etal-2013-decoding,
    title = "Decoding with Large-Scale Neural Language Models Improves Translation",
    author = "Vaswani, Ashish  and
      Zhao, Yinggong  and
      Fossum, Victoria  and
      Chiang, David",
    booktitle = "Proceedings of the 2013 Conference on Empirical Methods in Natural Language Processing",
    month = oct,
    year = "2013",
    address = "Seattle, Washington, USA",
    publisher = "Association for Computational Linguistics",
    pages = "1387--1392",
}
@ARTICLE{7050391,
  author={M. Sundermeyer and H. Ney and R. Schluter},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing},
  title={From Feedforward to Recurrent LSTM Neural Networks for Language Modeling},
  year={2015},
  volume={23},
  pages={517-529}
}
@inproceedings{bahdanau2014neural,
    title = {Neural Machine Translation by Jointly Learning to Align and Translate},
    author = {Bahdanau, Dzmitry and Cho, Kyunghyun and Bengio, Yoshua},
    booktitle  = {3rd International Conference on Learning Representations},
    month = {May},
    year = {2015},
    address = {San Diego, CA, USA},
    pubilsher = {OpenReview.net},
}
@inproceedings{kalchbrenner-blunsom-2013-recurrent,
    title = "Recurrent Continuous Translation Models",
    author = "Kalchbrenner, Nal  and
      Blunsom, Phil",
    booktitle = "Proceedings of the 2013 Conference on Empirical Methods in Natural Language Processing",
    month = oct,
    year = "2013",
    address = "Seattle, Washington, USA",
    publisher = "Association for Computational Linguistics",
    pages = "1700--1709",
}
@inproceedings{GehringAGYD17,
  title     = {Convolutional Sequence to Sequence Learning},
  author    = {Jonas Gehring and
               Michael Auli and
               David Grangier and
               Denis Yarats and
               Yann N. Dauphin},
  booktitle = {Proceedings of the 34th International Conference on Machine Learning,
               {ICML} 2017},
  month     = aug,
  year      = {2017},
  address   = {Sydney, NSW, Australia},
  publisher = {{PMLR}},
  pages     = {1243--1252},
}
@incollection{vaswani2017attention,
  title = {Attention is All you Need},
  author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, \L ukasz and Polosukhin, Illia},
  booktitle = {Advances in Neural Information Processing Systems 30},
  month=dec,
  year = {2017},
  address = "Long Beach, CA, USA",
  publisher = {Curran Associates, Inc.},
  pages = {5998--6008},
}
@article{brown-etal-1993-mathematics,
    title = "The Mathematics of Statistical Machine Translation: Parameter Estimation",
    author = "Brown, Peter F.  and
      Della Pietra, Stephen A.  and
      Della Pietra, Vincent J.  and
      Mercer, Robert L.",
    journal = "Computational Linguistics",
    volume = "19",
    number = "2",
    year = "1993",
    pages = "263--311",
}
@inproceedings{chen-goodman-1996-empirical,
    title = "An Empirical Study of Smoothing Techniques for Language Modeling",
    author = "Chen, Stanley F.  and
      Goodman, Joshua",
    booktitle = "34th Annual Meeting of the Association for Computational Linguistics",
    month = jun,
    year = "1996",
    address = "Santa Cruz, California, USA",
    publisher = "Association for Computational Linguistics",
    pages = "310--318",
}
@article{TillmannN03,
  author    = {Christoph Tillmann and Hermann Ney},
  title     = {Word Reordering and a Dynamic Programming Beam Search Algorithm for Statistical Machine Translation},
  journal   = {Computational Linguistics},
  volume    = {29},
  number    = {1},
  pages     = {97--133},
  year      = {2003},
}
@inproceedings{koehn-etal-2003-statistical,
    title = "Statistical Phrase-Based Translation",
    author = "Koehn, Philipp  and
      Och, Franz J.  and
      Marcu, Daniel",
    booktitle = "Proceedings of the 2003 Human Language Technology Conference of the North {A}merican Chapter of the Association for Computational Linguistics",
    year = "2003",
    pages = "127--133",
}
@InProceedings{10.1007/978-3-540-30194-3_13,
    title="Pharaoh: A Beam Search Decoder for Phrase-Based Statistical Machine Translation Models",
    author="Koehn, Philipp",
    editor="Frederking, Robert E.
    and Taylor, Kathryn B.",
    booktitle="Machine Translation: From Real Users to Research",
    month = "Sep",
    year="2004",
    address="Berlin, Heidelberg",
    pages="115--124",
}
@inproceedings{collins-koehn-kucerova:2005:ACL,
    title = "Clause Restructuring for Statistical Machine Translation",
    author = "Collins, Michael  and
      Koehn, Philipp  and
      Ku{\v{c}}erov{\'a}, Ivona",
    booktitle = "Proceedings of the 43rd Annual Meeting of the Association for Computational Linguistics ({ACL}{'}05)",
    month = jun,
    year = "2005",
    address = "Ann Arbor, Michigan",
    publisher = "Association for Computational Linguistics",
    pages = "531--540",
}
@article{hassan2018achieving,
  title={Achieving human parity on automatic chinese to english news translation},
  author={Hassan, Hany and Aue, Anthony and Chen, Chang and Chowdhary, Vishal and Clark, Jonathan and Federmann, Christian and Huang, Xuedong and Junczys-Dowmunt, Marcin and Lewis, William and Li, Mu and others},
  journal={arXiv preprint arXiv:1803.05567},
  year={2018}
}
@inproceedings{barrault-etal-2019-findings,
    title = "Findings of the 2019 Conference on Machine Translation ({WMT}19)",
    author = {Barrault, Lo{\"\i}c  and
      Bojar, Ond{\v{r}}ej  and
      Costa-juss{\`a}, Marta R.  and
      Federmann, Christian  and
      Fishel, Mark  and
      Graham, Yvette  and
      Haddow, Barry  and
      Huck, Matthias  and
      Koehn, Philipp  and
      Malmasi, Shervin  and
      Monz, Christof  and
      M{\"u}ller, Mathias  and
      Pal, Santanu  and
      Post, Matt  and
      Zampieri, Marcos},
    booktitle = "Proceedings of the Fourth Conference on Machine Translation (Volume 2: Shared Task Papers, Day 1)",
    month = aug,
    year = "2019",
    address = "Florence, Italy",
    publisher = "Association for Computational Linguistics",
    pages = "1--61",
}
@inproceedings{zheng2019dynamic,
    title = "Dynamic Past and Future for Neural Machine Translation",
    author = "Zheng, Zaixiang  and
      Huang, Shujian  and
      Tu, Zhaopeng  and
      Dai, Xin-Yu  and
      Chen, Jiajun",
    booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)",
    month = nov,
    year = "2019",
    address = "Hong Kong, China",
    publisher = "Association for Computational Linguistics",
    pages = "931--941",
}
@incollection{NIPS2017_6622,
  title = {Decoding with Value Networks for Neural Machine Translation},
  author = {He, Di and Lu, Hanqing and Xia, Yingce and Qin, Tao and Wang, Liwei and Liu, Tie-Yan},
  booktitle = {Advances in Neural Information Processing Systems 30},
  editor = {I. Guyon and U. V. Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
  month = dec,
  year = {2017},
  address = "Long Beach, CA, USA",
  publisher = {Curran Associates, Inc.},
  pages = {178--187},
}
@article{zheng-etal-2018-modeling,
    title = "Modeling Past and Future for Neural Machine Translation",
    author = "Zheng, Zaixiang  and
      Zhou, Hao  and
      Huang, Shujian  and
      Mou, Lili  and
      Dai, Xinyu  and
      Chen, Jiajun  and
      Tu, Zhaopeng",
    journal = "Transactions of the Association for Computational Linguistics",
    volume = "6",
    year = "2018",
    pages = "145--157",
}
@inproceedings{weng-etal-2017-neural,
    title = "Neural Machine Translation with Word Predictions",
    author = "Weng, Rongxiang  and
      Huang, Shujian  and
      Zheng, Zaixiang  and
      Dai, Xinyu  and
      Chen, Jiajun",
    booktitle = "Proceedings of the 2017 Conference on Empirical Methods in Natural Language Processing",
    month = sep,
    year = "2017",
    address = "Copenhagen, Denmark",
    publisher = "Association for Computational Linguistics",
    pages = "136--145",
}
@article{knight-1999-decoding,
    title = "Decoding complexity in word-replacement translation models",
    author = "Knight, Kevin",
    journal = "Computational Linguistics",
    volume = "25",
    number = "4",
    year = "1999",
    pages = "607--615",
}
@book{koehn2009statistical,
  title={Statistical machine translation},
  author={Koehn, Philipp},
  year={2009},
  publisher={Cambridge University Press}
}
@inproceedings{tu-etal-2016-modeling,
    title = "Modeling Coverage for Neural Machine Translation",
    author = "Tu, Zhaopeng  and
      Lu, Zhengdong  and
      Liu, Yang  and
      Liu, Xiaohua  and
      Li, Hang",
    booktitle = "Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = aug,
    year = "2016",
    address = "Berlin, Germany",
    publisher = "Association for Computational Linguistics",
    pages = "76--85",
}
@inproceedings{mi-etal-2016-coverage,
    title = "Coverage Embedding Models for Neural Machine Translation",
    author = "Mi, Haitao  and
      Sankaran, Baskaran  and
      Wang, Zhiguo  and
      Ittycheriah, Abe",
    booktitle = "Proceedings of the 2016 Conference on Empirical Methods in Natural Language Processing",
    month = nov,
    year = "2016",
    address = "Austin, Texas",
    publisher = "Association for Computational Linguistics",
    pages = "955--960",
}
@inproceedings{li-etal-2018-simple,
    title = "A Simple and Effective Approach to Coverage-Aware Neural Machine Translation",
    author = "Li, Yanyang  and
      Xiao, Tong  and
      Li, Yinqiao  and
      Wang, Qiang  and
      Xu, Changming  and
      Zhu, Jingbo",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)",
    month = jul,
    year = "2018",
    address = "Melbourne, Australia",
    publisher = "Association for Computational Linguistics",
    pages = "292--297",
}
@inproceedings{lin-etal-2018-deconvolution,
    title = "Deconvolution-Based Global Decoding for Neural Machine Translation",
    author = "Lin, Junyang  and
      Sun, Xu  and
      Ren, Xuancheng  and
      Ma, Shuming  and
      Su, Jinsong  and
      Su, Qi",
    booktitle = "Proceedings of the 27th International Conference on Computational Linguistics",
    month = aug,
    year = "2018",
    address = "Santa Fe, New Mexico, USA",
    publisher = "Association for Computational Linguistics",
    pages = "3260--3271",
}
@incollection{NIPS2017_6775,
  title = {Deliberation Networks: Sequence Generation Beyond One-Pass Decoding},
  author = {Xia, Yingce and Tian, Fei and Wu, Lijun and Lin, Jianxin and Qin, Tao and Yu, Nenghai and Liu, Tie-Yan},
  booktitle = {Advances in Neural Information Processing Systems 30},
  month = dec,
  year = {2017},
  address = "Long Beach, CA, USA",
  publisher = {Curran Associates, Inc.},
  pages = {1784--1794},
}
@article{zhou-etal-2019-synchronous,
    title = "Synchronous Bidirectional Neural Machine Translation",
    author = "Zhou, Long  and
      Zhang, Jiajun  and
      Zong, Chengqing",
    journal = "Transactions of the Association for Computational Linguistics",
    volume = "7",
    month = mar,
    year = "2019",
    pages = "91--105",
}
@inproceedings{li-etal-2018-target,
    title = "Target Foresight Based Attention for Neural Machine Translation",
    author = "Li, Xintong  and
      Liu, Lemao  and
      Tu, Zhaopeng  and
      Shi, Shuming  and
      Meng, Max",
    booktitle = "Proceedings of the 2018 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long Papers)",
    month = jun,
    year = "2018",
    address = "New Orleans, Louisiana",
    publisher = "Association for Computational Linguistics",
    pages = "1380--1390",
}
@inproceedings{hao-etal-2019-modeling,
    title = "Modeling Recurrence for Transformer",
    author = "Hao, Jie  and
      Wang, Xing  and
      Yang, Baosong  and
      Wang, Longyue  and
      Zhang, Jinfeng  and
      Tu, Zhaopeng",
    booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)",
    month = jun,
    year = "2019",
    address = "Minneapolis, Minnesota",
    publisher = "Association for Computational Linguistics",
    pages = "1198--1207",
}
@inproceedings{li-etal-2019-information,
    title = "Information Aggregation for Multi-Head Attention with Routing-by-Agreement",
    author = "Li, Jian  and
      Yang, Baosong  and
      Dou, Zi-Yi  and
      Wang, Xing  and
      Lyu, Michael R.  and
      Tu, Zhaopeng",
    booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)",
    month = jun,
    year = "2019",
    address = "Minneapolis, Minnesota",
    publisher = "Association for Computational Linguistics",
    pages = "3566--3575",
}
@inproceedings{li2020datadependent,
  title={Data-dependent Gaussian Prior Objective for Language Generation},
  author={Zuchao Li and Rui Wang and Kehai Chen and Masso Utiyama and Eiichiro Sumita and Zhuosheng Zhang and Hai Zhao},
  booktitle={International Conference on Learning Representations},
  month=apr,
  year={2020},
  address={Addis, Ababa},
  pubilsher = {OpenReview.net},
}
@inproceedings{MengTCWZYW18,
  author    = {Fandong Meng and
               Zhaopeng Tu and
               Yong Cheng and
               Haiyang Wu and
               Junjie Zhai and
               Yuekui Yang and
               Di Wang},
  title     = {Neural Machine Translation with Key-Value Memory-Augmented Attention},
  booktitle = {Proceedings of the Twenty-Seventh International Joint Conference on Artificial Intelligence},
  month     = jul,
  year      = {2018},
  address   = {Stockholm, Sweden},
  publisher = {ijcai.org},
  pages     = {2574--2580},
}
@inproceedings{ZhangSQLJW18,
  author    = {Xiangwen Zhang and
               Jinsong Su and
               Yue Qin and
               Yang Liu and
               Rongrong Ji and
               Hongji Wang},
  title     = {Asynchronous Bidirectional Decoding for Neural Machine Translation},
  booktitle = {Proceedings of the Thirty-Second {AAAI} Conference on Artificial Intelligence,
               (AAAI-18), the 30th innovative Applications of Artificial Intelligence
               (IAAI-18), and the 8th {AAAI} Symposium on Educational Advances in
               Artificial Intelligence (EAAI-18)},
  month     = feb,
  year      = {2018},
  address   = {New Orleans, Louisiana, USA},
  publisher = {{AAAI} Press},
  pages     = {5698--5705},
}
@inproceedings{geng-etal-2018-adaptive,
    title = "Adaptive Multi-pass Decoder for Neural Machine Translation",
    author = "Geng, Xinwei  and
      Feng, Xiaocheng  and
      Qin, Bing  and
      Liu, Ting",
    booktitle = "Proceedings of the 2018 Conference on Empirical Methods in Natural Language Processing",
    month = oct # "-" # nov,
    year = "2018",
    address = "Brussels, Belgium",
    publisher = "Association for Computational Linguistics",
    pages = "523--532",
}
@inproceedings{ZhangW0L0X19,
  author    = {Zhirui Zhang and
               Shuangzhi Wu and
               Shujie Liu and
               Mu Li and
               Ming Zhou and
               Tong Xu},
  title     = {Regularizing Neural Machine Translation by Target-Bidirectional Agreement},
  booktitle = {The Thirty-Third {AAAI} Conference on Artificial Intelligence, {AAAI}
               2019, The Thirty-First Innovative Applications of Artificial Intelligence
               Conference, {IAAI} 2019, The Ninth {AAAI} Symposium on Educational
               Advances in Artificial Intelligence, {EAAI} 2019},
  month     = jan,
  year      = {2019},
  address   = {Honolulu, Hawaii, USA},
  publisher = {{AAAI} Press},
  pages     = {443--450},
}
@incollection{NIPS2019_8861,
  title = {Neural Machine Translation with Soft Prototype},
  author = {Wang, Yiren and Xia, Yingce and Tian, Fei and Gao, Fei and Qin, Tao and Zhai, Cheng Xiang and Liu, Tie-Yan},
  booktitle = {Advances in Neural Information Processing Systems 32},
  month = dec,
  year = {2019},
  address = {Vancouver, BC, Canada},
  publisher = {Curran Associates, Inc.},
  pages = {6316--6325},
}
@inproceedings{SerdyukKSTPB18,
  author    = {Dmitriy Serdyuk and
               Nan Rosemary Ke and
               Alessandro Sordoni and
               Adam Trischler and
               Chris Pal and
               Yoshua Bengio},
  title     = {Twin Networks: Matching the Future for Sequence Generation},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018},
  month     = may,
  year      = {2018},
  address   = {Vancouver, BC, Canada},
  pubilsher = {OpenReview.net},
}
@article{LiMJ17,
  author    = {Jiwei Li and
               Will Monroe and
               Dan Jurafsky},
  title     = {Learning to Decode for Future Success},
  journal   = {CoRR},
  volume    = {abs/1701.06549},
  year      = {2017},
}
@inproceedings{BahdanauBXGLPCB17,
  author    = {Dzmitry Bahdanau and
               Philemon Brakel and
               Kelvin Xu and
               Anirudh Goyal and
               Ryan Lowe and
               Joelle Pineau and
               Aaron C. Courville and
               Yoshua Bengio},
  title     = {An Actor-Critic Algorithm for Sequence Prediction},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017},
  month     = apr,
  year      = {2017},
  address   = {Toulon, France},
  pubilsher = {OpenReview.net},
}
@inproceedings{KongTSHZ19,
  author    = {Xiang Kong and
               Zhaopeng Tu and
               Shuming Shi and
               Eduard H. Hovy and
               Tong Zhang},
  title     = {Neural Machine Translation with Adequacy-Oriented Learning},
  booktitle = {The Thirty-Third {AAAI} Conference on Artificial Intelligence, {AAAI}
               2019, The Thirty-First Innovative Applications of Artificial Intelligence
               Conference, {IAAI} 2019, The Ninth {AAAI} Symposium on Educational
               Advances in Artificial Intelligence, {EAAI} 2019},
  month     = jan,
  year      = {2019},
  address   = {Honolulu, Hawaii, USA},
  publisher = {{AAAI} Press},
  pages     = {6618--6625},
}
@ARTICLE{8811589,
  author={K. {Chen} and R. {Wang} and M. {Utiyama} and E. {Sumita} and T. {Zhao}},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing}, 
  title={Neural Machine Translation With Sentence-Level Topic Context}, 
  year={2019},
  volume={27},
  number={12},
  pages={1970-1984},
}
@ARTICLE{8550728,
  author={J. {Zhang} and Y. {Zhao} and H. {Li} and C. {Zong}},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing}, 
  title={Attention With Sparsity Regularization for Neural Machine Translation and Summarization}, 
  year={2019},
  volume={27},
  number={3},
  pages={507-518},
}
@ARTICLE{8421063,
  author={X. {Wang} and Z. {Tu} and M. {Zhang}},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing}, 
  title={Incorporating Statistical Machine Translation Word Knowledge Into Neural Machine Translation}, 
  year={2018},
  volume={26},
  number={12},
  pages={2255-2266},
}
@ARTICLE{7090970,
  author={R. {Wang} and H. {Zhao} and B. {Lu} and M. {Utiyama} and E. {Sumita}},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing}, 
  title={Bilingual Continuous-Space Language Model Growing for Statistical Machine Translation}, 
  year={2015},
  volume={23},
  number={7},
  pages={1209-1220},
}

@inproceedings{cao-attsum,
    title = "{A}tt{S}um: Joint Learning of Focusing and Summarization with Neural Attention",
    author = "Cao, Ziqiang  and
      Li, Wenjie  and
      Li, Sujian  and
      Wei, Furu  and
      Li, Yanran",
    booktitle = "Proceedings of {COLING} 2016, the 26th International Conference on Computational Linguistics: Technical Papers",
    month = dec,
    year = "2016",
    address = "Osaka, Japan",
    publisher = "The COLING 2016 Organizing Committee",
    url = "https://www.aclweb.org/anthology/C16-1053",
    pages = "547--556",
}

@article{svr,
title = "Applying regression models to query-focused multi-document summarization",
journal = "Information Processing \& Management",
volume = "47",
number = "2",
pages = "227 - 237",
year = "2011",
issn = "0306-4573",
doi = "https://doi.org/10.1016/j.ipm.2010.03.005",
url = "http://www.sciencedirect.com/science/article/pii/S0306457310000257",
author = "You Ouyang and Wenjie Li and Sujian Li and Qin Lu",
keywords = "Query-focused summarization, Support Vector Regression, Training data construction",
}

@inproceedings{prabhumoye2019towards,
author = {Prabhumoye, Shrimai and Quirk, Chris and Galley, Michel},
title = {Towards Content Transfer through Grounded Text Generation},
year = 2019,
booktitle = {Proc. of NAACL}
}

@incollection{transformer,
title = {Attention is All you Need},
author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, \L ukasz and Polosukhin, Illia},
booktitle = {Advances in Neural Information Processing Systems 30},
editor = {I. Guyon and U. V. Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
pages = {5998--6008},
year = {2017},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/7181-attention-is-all-you-need.pdf}
}

@InProceedings{kingma:adam,
author = {Kingma, Diederick P and Ba, Jimmy},
title = {Adam: A method for stochastic optimization},
booktitle = { International Conference on Learning Representations (ICLR) },
year = {2015}
}


@inproceedings{bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  booktitle={Human Language Technologies: The 2019 Annual Conference of the North American Chapter of the Association for Computational Linguistics},
  year={2019},
}

@inproceedings{wikisum,
title={Generating Wikipedia by Summarizing Long Sequences},
author={Peter J. Liu and Mohammad Saleh and Etienne Pot and Ben Goodrich and Ryan Sepassi and Lukasz Kaiser and Noam Shazeer},
booktitle={International Conference on Learning Representations},
year={2018},
url={https://openreview.net/forum?id=Hyg0vbWC-},
}

@inproceedings{logist_regression,
  title={Using supervised bigram-based ILP for extractive summarization},
  author={Li, Chen and Qian, Xian and Liu, Yang},
  booktitle={Proceedings of the 51st Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  volume={1},
  pages={1004--1013},
  year={2013}
}

@inproceedings{crf,
    title = "A Skip-Chain Conditional Random Field for Ranking Meeting Utterances by Importance",
    author = "Galley, Michel",
    booktitle = "Proceedings of the 2006 Conference on Empirical Methods in Natural Language Processing",
    month = jul,
    year = "2006",
    address = "Sydney, Australia",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/W06-1643",
    pages = "364--372",
}

@inproceedings{Ren-crsum,
 author = {Ren, Pengjie and Chen, Zhumin and Ren, Zhaochun and Wei, Furu and Ma, Jun and de Rijke, Maarten},
 title = {Leveraging Contextual Sentence Relations for Extractive Summarization Using a Neural Attention Model},
 booktitle = {Proceedings of the 40th International ACM SIGIR Conference on Research and Development in Information Retrieval},
 series = {SIGIR '17},
 year = {2017},
 isbn = {978-1-4503-5022-8},
 location = {Shinjuku, Tokyo, Japan},
 pages = {95--104},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/3077136.3080792},
 doi = {10.1145/3077136.3080792},
 acmid = {3080792},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {contextual sentence relation, extractive summarization, neural network},
} 

@inproceedings{zhou-etal-2018-neural-document,
    title = "Neural Document Summarization by Jointly Learning to Score and Select Sentences",
    author = "Zhou, Qingyu  and
      Yang, Nan  and
      Wei, Furu  and
      Huang, Shaohan  and
      Zhou, Ming  and
      Zhao, Tiejun",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2018",
    address = "Melbourne, Australia",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P18-1061",
    pages = "654--663",
}




@inproceedings{lin-2004-rouge,
    title = "{ROUGE}: A Package for Automatic Evaluation of Summaries",
    author = "Lin, Chin-Yew",
    booktitle = "Text Summarization Branches Out: Proceedings of the {ACL}-04 Workshop",
    month = jul,
    year = "2004",
    address = "Barcelona, Spain",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/W04-1013",
    pages = "74--81",
}

@inproceedings{duc05overview,
  title={Overview of DUC 2005},
  author={Dang, Hoa Trang},
  booktitle={Proceedings of the document understanding conference},
  volume={2005},
  pages={1--12},
  year={2005},
}

@InProceedings{ilp,
author="McDonald, Ryan",
editor="Amati, Giambattista
and Carpineto, Claudio
and Romano, Giovanni",
title="A Study of Global Inference Algorithms in Multi-document Summarization",
booktitle="Advances in Information Retrieval",
year="2007",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="557--564",
}

@article{erkan2004lexrank,
  title={Lexrank: Graph-based lexical centrality as salience in text summarization},
  author={Erkan, G{\"u}nes and Radev, Dragomir R},
  journal={Journal of artificial intelligence research},
  volume={22},
  pages={457--479},
  year={2004}
}

@InProceedings{qfs_graph,
	author = {Xiaojun Wan and Jianguo Xiao},
	title = {Graph-Based Multi-Modality Learning for Topic-Focused Multi-Document Summarization},
	booktitle = {International Joint Conference on Artificial Intelligence},
	year = {2009},
	keywords = {multi-document summarization; manifold-ranking; multi-modality learning},
	url = {https://www.aaai.org/ocs/index.php/IJCAI/IJCAI-09/paper/view/650}
}

@inproceedings{wan-2008-exploration-graph,
    title = "An Exploration of Document Impact on Graph-Based Multi-Document Summarization",
    author = "Wan, Xiaojun",
    booktitle = "Proceedings of the 2008 Conference on Empirical Methods in Natural Language Processing",
    month = oct,
    year = "2008",
    address = "Honolulu, Hawaii",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/D08-1079",
    pages = "755--762",
}

@inproceedings{mmr,
 author = {Carbonell, Jaime and Goldstein, Jade},
 title = {The Use of MMR, Diversity-based Reranking for Reordering Documents and Producing Summaries},
 booktitle = {Proceedings of the 21st Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
 series = {SIGIR '98},
 year = {1998},
 isbn = {1-58113-015-5},
 location = {Melbourne, Australia},
 pages = {335--336},
 numpages = {2},
 url = {http://doi.acm.org/10.1145/290941.291025},
 doi = {10.1145/290941.291025},
 acmid = {291025},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{lin2010multi,
  title={Multi-document summarization via budgeted maximization of submodular functions},
  author={Lin, Hui and Bilmes, Jeff},
  booktitle={Human Language Technologies: The 2010 Annual Conference of the North American Chapter of the Association for Computational Linguistics},
  pages={912--920},
  year={2010}
}

@inproceedings{ft-bert-extractive,
    title = "Text Summarization with Pretrained Encoders",
    author = "Liu, Yang  and
      Lapata, Mirella",
    booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)",
    month = nov,
    year = "2019",
    address = "Hong Kong, China",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D19-1387",
    doi = "10.18653/v1/D19-1387",
    pages = "3730--3740",
}

@inproceedings{c14-1001,
  author =	"harper, mary",
  title = 	"learning from @inproceedings{klein-etal:2017:acl-2017-system-demonstrations,
    title = "{o}pen{nmt}: open-source toolkit for neural machine translation",
    author = "klein, guillaume  and
      kim, yoon  and
      deng, yuntian  and
      senellart, jean  and
      rush, alexander",
    booktitle = "proceedings of {acl} 2017, system demonstrations",
    month = jul,
    year = "2017",
    address = "vancouver, canada",
    publisher = "association for computational linguistics",
    pages = "67--72",
}
@inproceedings{ott2019fairseq,
    title = "fairseq: a fast, extensible toolkit for sequence modeling",
    author = "ott, myle  and
      edunov, sergey  and
      baevski, alexei  and
      fan, angela  and
      gross, sam  and
      ng, nathan  and
      grangier, david  and
      auli, michael",
    booktitle = "proceedings of the 2019 conference of the north {a}merican chapter of the association for computational linguistics (demonstrations)",
    month = jun,
    year = "2019",
    address = "minneapolis, minnesota",
    publisher = "association for computational linguistics",
    pages = "48--53",
}
@inproceedings{sennrich-haddow-birch:2016:p16-12,
    title = "neural machine translation of rare words with subword units",
    author = "sennrich, rico  and
      haddow, barry  and
      birch, alexandra",
    booktitle = "proceedings of the 54th annual meeting of the association for computational linguistics (volume 1: long papers)",
    month = aug,
    year = "2016",
    address = "berlin, germany",
    publisher = "association for computational linguistics",
    pages = "1715--1725",
}
@inproceedings{kingma2014adam,
  title = "adam: {a} method for stochastic optimization",
  author = "diederik p. kingma and
               jimmy ba",
  booktitle = "3rd international conference on learning representations",
  month = may,
  year = "2015",
  address = "san diego, ca, usa",
  pubilsher = {openreview.net},
}
@inproceedings{he2016deep,
  title="deep residual learning for image recognition",
  author="he, kaiming and zhang, xiangyu and ren, shaoqing and sun, jian",
  booktitle="proceedings of the ieee conference on computer vision and pattern recognition",
  month=jun,
  year="2016",
  address="las vegas, nv, usa",
  publisher="ieee computer society",
  pages="770--778",
}
@article{ba2016layer,
  title="layer normalization",
  author="ba, jimmy lei and kiros, jamie ryan and hinton, geoffrey e",
  journal="arxiv preprint arxiv:1607.06450",
  month = jul,
  year="2016",
}
@inproceedings{cho2014learning,
    title = "learning phrase representations using {rnn} encoder{--}decoder for statistical machine translation",
    author = {cho, kyunghyun  and
      van merri{\"e}nboer, bart  and
      gulcehre, caglar  and
      bahdanau, dzmitry  and
      bougares, fethi  and
      schwenk, holger  and
      bengio, yoshua},
    booktitle = "proceedings of the 2014 conference on empirical methods in natural language processing ({emnlp})",
    month = oct,
    year = "2014",
    address = "doha, qatar",
    publisher = "association for computational linguistics",
    pages = "1724--1734",
}
@article{10.5555/944919.944966,
    author = {bengio, yoshua and ducharme, r\'{e}jean and vincent, pascal and janvin, christian},
    title = {a neural probabilistic language model},
    year = {2003},
    volume = {3},
    issn = {1532-4435},
    journal = {journal of machine learning research},
    month = {march},
    pages = {1137–1155},
    numpages = {19}
}
@inproceedings{mikolov2010recurrent,
  author={mikolov, tomas and karafi{\'a}t, martin and burget, lukas and cernock{\`y}, jan and khudanpur, sanjeev},
  title={recurrent neural network based language model},
  booktitle={proceedings of the conference of the international speech communication association},
  year={2010},
  address={makuhari, chiba, japan},
  pages={1045--1048}
}
@inproceedings{vaswani-etal-2013-decoding,
    title = "decoding with large-scale neural language models improves translation",
    author = "vaswani, ashish  and
      zhao, yinggong  and
      fossum, victoria  and
      chiang, david",
    booktitle = "proceedings of the 2013 conference on empirical methods in natural language processing",
    month = oct,
    year = "2013",
    address = "seattle, washington, usa",
    publisher = "association for computational linguistics",
    pages = "1387--1392",
}
@article{7050391,
  author={m. sundermeyer and h. ney and r. schluter},
  journal={ieee/acm transactions on audio, speech, and language processing},
  title={from feedforward to recurrent lstm neural networks for language modeling},
  year={2015},
  volume={23},
  pages={517-529}
}
@inproceedings{bahdanau2014neural,
    title = {neural machine translation by jointly learning to align and translate},
    author = {bahdanau, dzmitry and cho, kyunghyun and bengio, yoshua},
    booktitle  = {3rd international conference on learning representations},
    month = {may},
    year = {2015},
    address = {san diego, ca, usa},
    pubilsher = {openreview.net},
}
@inproceedings{kalchbrenner-blunsom-2013-recurrent,
    title = "recurrent continuous translation models",
    author = "kalchbrenner, nal  and
      blunsom, phil",
    booktitle = "proceedings of the 2013 conference on empirical methods in natural language processing",
    month = oct,
    year = "2013",
    address = "seattle, washington, usa",
    publisher = "association for computational linguistics",
    pages = "1700--1709",
}
@inproceedings{gehringagyd17,
  title     = {convolutional sequence to sequence learning},
  author    = {jonas gehring and
               michael auli and
               david grangier and
               denis yarats and
               yann n. dauphin},
  booktitle = {proceedings of the 34th international conference on machine learning,
               {icml} 2017},
  month     = aug,
  year      = {2017},
  address   = {sydney, nsw, australia},
  publisher = {{pmlr}},
  pages     = {1243--1252},
}
@incollection{vaswani2017attention,
  title = {attention is all you need},
  author = {vaswani, ashish and shazeer, noam and parmar, niki and uszkoreit, jakob and jones, llion and gomez, aidan n and kaiser, \l ukasz and polosukhin, illia},
  booktitle = {advances in neural information processing systems 30},
  month=dec,
  year = {2017},
  address = "long beach, ca, usa",
  publisher = {curran associates, inc.},
  pages = {5998--6008},
}
@article{brown-etal-1993-mathematics,
    title = "the mathematics of statistical machine translation: parameter estimation",
    author = "brown, peter f.  and
      della pietra, stephen a.  and
      della pietra, vincent j.  and
      mercer, robert l.",
    journal = "computational linguistics",
    volume = "19",
    number = "2",
    year = "1993",
    pages = "263--311",
}
@inproceedings{chen-goodman-1996-empirical,
    title = "an empirical study of smoothing techniques for language modeling",
    author = "chen, stanley f.  and
      goodman, joshua",
    booktitle = "34th annual meeting of the association for computational linguistics",
    month = jun,
    year = "1996",
    address = "santa cruz, california, usa",
    publisher = "association for computational linguistics",
    pages = "310--318",
}
@article{tillmannn03,
  author    = {christoph tillmann and hermann ney},
  title     = {word reordering and a dynamic programming beam search algorithm for statistical machine translation},
  journal   = {computational linguistics},
  volume    = {29},
  number    = {1},
  pages     = {97--133},
  year      = {2003},
}
@inproceedings{koehn-etal-2003-statistical,
    title = "statistical phrase-based translation",
    author = "koehn, philipp  and
      och, franz j.  and
      marcu, daniel",
    booktitle = "proceedings of the 2003 human language technology conference of the north {a}merican chapter of the association for computational linguistics",
    year = "2003",
    pages = "127--133",
}
@inproceedings{10.1007/978-3-540-30194-3_13,
    title="pharaoh: a beam search decoder for phrase-based statistical machine translation models",
    author="koehn, philipp",
    editor="frederking, robert e.
    and taylor, kathryn b.",
    booktitle="machine translation: from real users to research",
    month = "sep",
    year="2004",
    address="berlin, heidelberg",
    pages="115--124",
}
@inproceedings{collins-koehn-kucerova:2005:acl,
    title = "clause restructuring for statistical machine translation",
    author = "collins, michael  and
      koehn, philipp  and
      ku{\v{c}}erov{\'a}, ivona",
    booktitle = "proceedings of the 43rd annual meeting of the association for computational linguistics ({acl}{'}05)",
    month = jun,
    year = "2005",
    address = "ann arbor, michigan",
    publisher = "association for computational linguistics",
    pages = "531--540",
}
@article{hassan2018achieving,
  title={achieving human parity on automatic chinese to english news translation},
  author={hassan, hany and aue, anthony and chen, chang and chowdhary, vishal and clark, jonathan and federmann, christian and huang, xuedong and junczys-dowmunt, marcin and lewis, william and li, mu and others},
  journal={arxiv preprint arxiv:1803.05567},
  year={2018}
}
@inproceedings{barrault-etal-2019-findings,
    title = "findings of the 2019 conference on machine translation ({wmt}19)",
    author = {barrault, lo{\"\i}c  and
      bojar, ond{\v{r}}ej  and
      costa-juss{\`a}, marta r.  and
      federmann, christian  and
      fishel, mark  and
      graham, yvette  and
      haddow, barry  and
      huck, matthias  and
      koehn, philipp  and
      malmasi, shervin  and
      monz, christof  and
      m{\"u}ller, mathias  and
      pal, santanu  and
      post, matt  and
      zampieri, marcos},
    booktitle = "proceedings of the fourth conference on machine translation (volume 2: shared task papers, day 1)",
    month = aug,
    year = "2019",
    address = "florence, italy",
    publisher = "association for computational linguistics",
    pages = "1--61",
}
@inproceedings{zheng2019dynamic,
    title = "dynamic past and future for neural machine translation",
    author = "zheng, zaixiang  and
      huang, shujian  and
      tu, zhaopeng  and
      dai, xin-yu  and
      chen, jiajun",
    booktitle = "proceedings of the 2019 conference on empirical methods in natural language processing and the 9th international joint conference on natural language processing (emnlp-ijcnlp)",
    month = nov,
    year = "2019",
    address = "hong kong, china",
    publisher = "association for computational linguistics",
    pages = "931--941",
}
@incollection{nips2017_6622,
  title = {decoding with value networks for neural machine translation},
  author = {he, di and lu, hanqing and xia, yingce and qin, tao and wang, liwei and liu, tie-yan},
  booktitle = {advances in neural information processing systems 30},
  editor = {i. guyon and u. v. luxburg and s. bengio and h. wallach and r. fergus and s. vishwanathan and r. garnett},
  month = dec,
  year = {2017},
  address = "long beach, ca, usa",
  publisher = {curran associates, inc.},
  pages = {178--187},
}
@article{zheng-etal-2018-modeling,
    title = "modeling past and future for neural machine translation",
    author = "zheng, zaixiang  and
      zhou, hao  and
      huang, shujian  and
      mou, lili  and
      dai, xinyu  and
      chen, jiajun  and
      tu, zhaopeng",
    journal = "transactions of the association for computational linguistics",
    volume = "6",
    year = "2018",
    pages = "145--157",
}
@inproceedings{weng-etal-2017-neural,
    title = "neural machine translation with word predictions",
    author = "weng, rongxiang  and
      huang, shujian  and
      zheng, zaixiang  and
      dai, xinyu  and
      chen, jiajun",
    booktitle = "proceedings of the 2017 conference on empirical methods in natural language processing",
    month = sep,
    year = "2017",
    address = "copenhagen, denmark",
    publisher = "association for computational linguistics",
    pages = "136--145",
}
@article{knight-1999-decoding,
    title = "decoding complexity in word-replacement translation models",
    author = "knight, kevin",
    journal = "computational linguistics",
    volume = "25",
    number = "4",
    year = "1999",
    pages = "607--615",
}
@book{koehn2009statistical,
  title={statistical machine translation},
  author={koehn, philipp},
  year={2009},
  publisher={cambridge university press}
}
@inproceedings{tu-etal-2016-modeling,
    title = "modeling coverage for neural machine translation",
    author = "tu, zhaopeng  and
      lu, zhengdong  and
      liu, yang  and
      liu, xiaohua  and
      li, hang",
    booktitle = "proceedings of the 54th annual meeting of the association for computational linguistics (volume 1: long papers)",
    month = aug,
    year = "2016",
    address = "berlin, germany",
    publisher = "association for computational linguistics",
    pages = "76--85",
}
@inproceedings{mi-etal-2016-coverage,
    title = "coverage embedding models for neural machine translation",
    author = "mi, haitao  and
      sankaran, baskaran  and
      wang, zhiguo  and
      ittycheriah, abe",
    booktitle = "proceedings of the 2016 conference on empirical methods in natural language processing",
    month = nov,
    year = "2016",
    address = "austin, texas",
    publisher = "association for computational linguistics",
    pages = "955--960",
}
@inproceedings{li-etal-2018-simple,
    title = "a simple and effective approach to coverage-aware neural machine translation",
    author = "li, yanyang  and
      xiao, tong  and
      li, yinqiao  and
      wang, qiang  and
      xu, changming  and
      zhu, jingbo",
    booktitle = "proceedings of the 56th annual meeting of the association for computational linguistics (volume 2: short papers)",
    month = jul,
    year = "2018",
    address = "melbourne, australia",
    publisher = "association for computational linguistics",
    pages = "292--297",
}
@inproceedings{lin-etal-2018-deconvolution,
    title = "deconvolution-based global decoding for neural machine translation",
    author = "lin, junyang  and
      sun, xu  and
      ren, xuancheng  and
      ma, shuming  and
      su, jinsong  and
      su, qi",
    booktitle = "proceedings of the 27th international conference on computational linguistics",
    month = aug,
    year = "2018",
    address = "santa fe, new mexico, usa",
    publisher = "association for computational linguistics",
    pages = "3260--3271",
}
@incollection{nips2017_6775,
  title = {deliberation networks: sequence generation beyond one-pass decoding},
  author = {xia, yingce and tian, fei and wu, lijun and lin, jianxin and qin, tao and yu, nenghai and liu, tie-yan},
  booktitle = {advances in neural information processing systems 30},
  month = dec,
  year = {2017},
  address = "long beach, ca, usa",
  publisher = {curran associates, inc.},
  pages = {1784--1794},
}
@article{zhou-etal-2019-synchronous,
    title = "synchronous bidirectional neural machine translation",
    author = "zhou, long  and
      zhang, jiajun  and
      zong, chengqing",
    journal = "transactions of the association for computational linguistics",
    volume = "7",
    month = mar,
    year = "2019",
    pages = "91--105",
}
@inproceedings{li-etal-2018-target,
    title = "target foresight based attention for neural machine translation",
    author = "li, xintong  and
      liu, lemao  and
      tu, zhaopeng  and
      shi, shuming  and
      meng, max",
    booktitle = "proceedings of the 2018 conference of the north {a}merican chapter of the association for computational linguistics: human language technologies, volume 1 (long papers)",
    month = jun,
    year = "2018",
    address = "new orleans, louisiana",
    publisher = "association for computational linguistics",
    pages = "1380--1390",
}
@inproceedings{hao-etal-2019-modeling,
    title = "modeling recurrence for transformer",
    author = "hao, jie  and
      wang, xing  and
      yang, baosong  and
      wang, longyue  and
      zhang, jinfeng  and
      tu, zhaopeng",
    booktitle = "proceedings of the 2019 conference of the north {a}merican chapter of the association for computational linguistics: human language technologies, volume 1 (long and short papers)",
    month = jun,
    year = "2019",
    address = "minneapolis, minnesota",
    publisher = "association for computational linguistics",
    pages = "1198--1207",
}
@inproceedings{li-etal-2019-information,
    title = "information aggregation for multi-head attention with routing-by-agreement",
    author = "li, jian  and
      yang, baosong  and
      dou, zi-yi  and
      wang, xing  and
      lyu, michael r.  and
      tu, zhaopeng",
    booktitle = "proceedings of the 2019 conference of the north {a}merican chapter of the association for computational linguistics: human language technologies, volume 1 (long and short papers)",
    month = jun,
    year = "2019",
    address = "minneapolis, minnesota",
    publisher = "association for computational linguistics",
    pages = "3566--3575",
}
@inproceedings{li2020datadependent,
  title={data-dependent gaussian prior objective for language generation},
  author={zuchao li and rui wang and kehai chen and masso utiyama and eiichiro sumita and zhuosheng zhang and hai zhao},
  booktitle={international conference on learning representations},
  month=apr,
  year={2020},
  address={addis, ababa},
  pubilsher = {openreview.net},
}
@inproceedings{mengtcwzyw18,
  author    = {fandong meng and
               zhaopeng tu and
               yong cheng and
               haiyang wu and
               junjie zhai and
               yuekui yang and
               di wang},
  title     = {neural machine translation with key-value memory-augmented attention},
  booktitle = {proceedings of the twenty-seventh international joint conference on artificial intelligence},
  month     = jul,
  year      = {2018},
  address   = {stockholm, sweden},
  publisher = {ijcai.org},
  pages     = {2574--2580},
}
@inproceedings{zhangsqljw18,
  author    = {xiangwen zhang and
               jinsong su and
               yue qin and
               yang liu and
               rongrong ji and
               hongji wang},
  title     = {asynchronous bidirectional decoding for neural machine translation},
  booktitle = {proceedings of the thirty-second {aaai} conference on artificial intelligence,
               (aaai-18), the 30th innovative applications of artificial intelligence
               (iaai-18), and the 8th {aaai} symposium on educational advances in
               artificial intelligence (eaai-18)},
  month     = feb,
  year      = {2018},
  address   = {new orleans, louisiana, usa},
  publisher = {{aaai} press},
  pages     = {5698--5705},
}
@inproceedings{geng-etal-2018-adaptive,
    title = "adaptive multi-pass decoder for neural machine translation",
    author = "geng, xinwei  and
      feng, xiaocheng  and
      qin, bing  and
      liu, ting",
    booktitle = "proceedings of the 2018 conference on empirical methods in natural language processing",
    month = oct # "-" # nov,
    year = "2018",
    address = "brussels, belgium",
    publisher = "association for computational linguistics",
    pages = "523--532",
}
@inproceedings{zhangw0l0x19,
  author    = {zhirui zhang and
               shuangzhi wu and
               shujie liu and
               mu li and
               ming zhou and
               tong xu},
  title     = {regularizing neural machine translation by target-bidirectional agreement},
  booktitle = {the thirty-third {aaai} conference on artificial intelligence, {aaai}
               2019, the thirty-first innovative applications of artificial intelligence
               conference, {iaai} 2019, the ninth {aaai} symposium on educational
               advances in artificial intelligence, {eaai} 2019},
  month     = jan,
  year      = {2019},
  address   = {honolulu, hawaii, usa},
  publisher = {{aaai} press},
  pages     = {443--450},
}
@incollection{nips2019_8861,
  title = {neural machine translation with soft prototype},
  author = {wang, yiren and xia, yingce and tian, fei and gao, fei and qin, tao and zhai, cheng xiang and liu, tie-yan},
  booktitle = {advances in neural information processing systems 32},
  month = dec,
  year = {2019},
  address = {vancouver, bc, canada},
  publisher = {curran associates, inc.},
  pages = {6316--6325},
}
@inproceedings{serdyukkstpb18,
  author    = {dmitriy serdyuk and
               nan rosemary ke and
               alessandro sordoni and
               adam trischler and
               chris pal and
               yoshua bengio},
  title     = {twin networks: matching the future for sequence generation},
  booktitle = {6th international conference on learning representations, {iclr} 2018},
  month     = may,
  year      = {2018},
  address   = {vancouver, bc, canada},
  pubilsher = {openreview.net},
}
@article{limj17,
  author    = {jiwei li and
               will monroe and
               dan jurafsky},
  title     = {learning to decode for future success},
  journal   = {corr},
  volume    = {abs/1701.06549},
  year      = {2017},
}
@inproceedings{bahdanaubxglpcb17,
  author    = {dzmitry bahdanau and
               philemon brakel and
               kelvin xu and
               anirudh goyal and
               ryan lowe and
               joelle pineau and
               aaron c. courville and
               yoshua bengio},
  title     = {an actor-critic algorithm for sequence prediction},
  booktitle = {5th international conference on learning representations, {iclr} 2017},
  month     = apr,
  year      = {2017},
  address   = {toulon, france},
  pubilsher = {openreview.net},
}
@inproceedings{kongtshz19,
  author    = {xiang kong and
               zhaopeng tu and
               shuming shi and
               eduard h. hovy and
               tong zhang},
  title     = {neural machine translation with adequacy-oriented learning},
  booktitle = {the thirty-third {aaai} conference on artificial intelligence, {aaai}
               2019, the thirty-first innovative applications of artificial intelligence
               conference, {iaai} 2019, the ninth {aaai} symposium on educational
               advances in artificial intelligence, {eaai} 2019},
  month     = jan,
  year      = {2019},
  address   = {honolulu, hawaii, usa},
  publisher = {{aaai} press},
  pages     = {6618--6625},
}
@article{8811589,
  author={k. {chen} and r. {wang} and m. {utiyama} and e. {sumita} and t. {zhao}},
  journal={ieee/acm transactions on audio, speech, and language processing}, 
  title={neural machine translation with sentence-level topic context}, 
  year={2019},
  volume={27},
  number={12},
  pages={1970-1984},
}
@article{8550728,
  author={j. {zhang} and y. {zhao} and h. {li} and c. {zong}},
  journal={ieee/acm transactions on audio, speech, and language processing}, 
  title={attention with sparsity regularization for neural machine translation and summarization}, 
  year={2019},
  volume={27},
  number={3},
  pages={507-518},
}
@article{8421063,
  author={x. {wang} and z. {tu} and m. {zhang}},
  journal={ieee/acm transactions on audio, speech, and language processing}, 
  title={incorporating statistical machine translation word knowledge into neural machine translation}, 
  year={2018},
  volume={26},
  number={12},
  pages={2255-2266},
}
@article{7090970,
  author={r. {wang} and h. {zhao} and b. {lu} and m. {utiyama} and e. {sumita}},
  journal={ieee/acm transactions on audio, speech, and language processing}, 
  title={bilingual continuous-space language model growing for statistical machine translation}, 
  year={2015},
  volume={23},
  number={7},
  pages={1209-1220},
}

@inproceedings{cao-attsum,
    title = "{a}tt{s}um: joint learning of focusing and summarization with neural attention",
    author = "cao, ziqiang  and
      li, wenjie  and
      li, sujian  and
      wei, furu  and
      li, yanran",
    booktitle = "proceedings of {coling} 2016, the 26th international conference on computational linguistics: technical papers",
    month = dec,
    year = "2016",
    address = "osaka, japan",
    publisher = "the coling 2016 organizing committee",
    url = "https://www.aclweb.org/anthology/c16-1053",
    pages = "547--556",
}

@article{svr,
title = "applying regression models to query-focused multi-document summarization",
journal = "information processing \& management",
volume = "47",
number = "2",
pages = "227 - 237",
year = "2011",
issn = "0306-4573",
doi = "https://doi.org/10.1016/j.ipm.2010.03.005",
url = "http://www.sciencedirect.com/science/article/pii/s0306457310000257",
author = "you ouyang and wenjie li and sujian li and qin lu",
keywords = "query-focused summarization, support vector regression, training data construction",
}

@inproceedings{prabhumoye2019towards,
author = {prabhumoye, shrimai and quirk, chris and galley, michel},
title = {towards content transfer through grounded text generation},
year = 2019,
booktitle = {proc. of naacl}
}

@incollection{transformer,
title = {attention is all you need},
author = {vaswani, ashish and shazeer, noam and parmar, niki and uszkoreit, jakob and jones, llion and gomez, aidan n and kaiser, \l ukasz and polosukhin, illia},
booktitle = {advances in neural information processing systems 30},
editor = {i. guyon and u. v. luxburg and s. bengio and h. wallach and r. fergus and s. vishwanathan and r. garnett},
pages = {5998--6008},
year = {2017},
publisher = {curran associates, inc.},
url = {http://papers.nips.cc/paper/7181-attention-is-all-you-need.pdf}
}

@inproceedings{kingma:adam,
author = {kingma, diederick p and ba, jimmy},
title = {adam: a method for stochastic optimization},
booktitle = { international conference on learning representations (iclr) },
year = {2015}
}


@inproceedings{bert,
  title={bert: pre-training of deep bidirectional transformers for language understanding},
  author={devlin, jacob and chang, ming-wei and lee, kenton and toutanova, kristina},
  booktitle={human language technologies: the 2019 annual conference of the north american chapter of the association for computational linguistics},
  year={2019},
}

@inproceedings{wikisum,
title={generating wikipedia by summarizing long sequences},
author={peter j. liu and mohammad saleh and etienne pot and ben goodrich and ryan sepassi and lukasz kaiser and noam shazeer},
booktitle={international conference on learning representations},
year={2018},
url={https://openreview.net/forum?id=hyg0vbwc-},
}

@inproceedings{logist_regression,
  title={using supervised bigram-based ilp for extractive summarization},
  author={li, chen and qian, xian and liu, yang},
  booktitle={proceedings of the 51st annual meeting of the association for computational linguistics (volume 1: long papers)},
  volume={1},
  pages={1004--1013},
  year={2013}
}

@inproceedings{crf,
    title = "a skip-chain conditional random field for ranking meeting utterances by importance",
    author = "galley, michel",
    booktitle = "proceedings of the 2006 conference on empirical methods in natural language processing",
    month = jul,
    year = "2006",
    address = "sydney, australia",
    publisher = "association for computational linguistics",
    url = "https://www.aclweb.org/anthology/w06-1643",
    pages = "364--372",
}

@inproceedings{ren-crsum,
 author = {ren, pengjie and chen, zhumin and ren, zhaochun and wei, furu and ma, jun and de rijke, maarten},
 title = {leveraging contextual sentence relations for extractive summarization using a neural attention model},
 booktitle = {proceedings of the 40th international acm sigir conference on research and development in information retrieval},
 series = {sigir '17},
 year = {2017},
 isbn = {978-1-4503-5022-8},
 location = {shinjuku, tokyo, japan},
 pages = {95--104},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/3077136.3080792},
 doi = {10.1145/3077136.3080792},
 acmid = {3080792},
 publisher = {acm},
 address = {new york, ny, usa},
 keywords = {contextual sentence relation, extractive summarization, neural network},
} 

@inproceedings{zhou-etal-2018-neural-document,
    title = "neural document summarization by jointly learning to score and select sentences",
    author = "zhou, qingyu  and
      yang, nan  and
      wei, furu  and
      huang, shaohan  and
      zhou, ming  and
      zhao, tiejun",
    booktitle = "proceedings of the 56th annual meeting of the association for computational linguistics (volume 1: long papers)",
    month = jul,
    year = "2018",
    address = "melbourne, australia",
    publisher = "association for computational linguistics",
    url = "https://www.aclweb.org/anthology/p18-1061",
    pages = "654--663",
}




@inproceedings{lin-2004-rouge,
    title = "{rouge}: a package for automatic evaluation of summaries",
    author = "lin, chin-yew",
    booktitle = "text summarization branches out: proceedings of the {acl}-04 workshop",
    month = jul,
    year = "2004",
    address = "barcelona, spain",
    publisher = "association for computational linguistics",
    url = "https://www.aclweb.org/anthology/w04-1013",
    pages = "74--81",
}

@inproceedings{duc05overview,
  title={overview of duc 2005},
  author={dang, hoa trang},
  booktitle={proceedings of the document understanding conference},
  volume={2005},
  pages={1--12},
  year={2005},
}

@inproceedings{ilp,
author="mcdonald, ryan",
editor="amati, giambattista
and carpineto, claudio
and romano, giovanni",
title="a study of global inference algorithms in multi-document summarization",
booktitle="advances in information retrieval",
year="2007",
publisher="springer berlin heidelberg",
address="berlin, heidelberg",
pages="557--564",
}

@article{erkan2004lexrank,
  title={lexrank: graph-based lexical centrality as salience in text summarization},
  author={erkan, g{\"u}nes and radev, dragomir r},
  journal={journal of artificial intelligence research},
  volume={22},
  pages={457--479},
  year={2004}
}

@inproceedings{qfs_graph,
	author = {xiaojun wan and jianguo xiao},
	title = {graph-based multi-modality learning for topic-focused multi-document summarization},
	booktitle = {international joint conference on artificial intelligence},
	year = {2009},
	keywords = {multi-document summarization; manifold-ranking; multi-modality learning},
	url = {https://www.aaai.org/ocs/index.php/ijcai/ijcai-09/paper/view/650}
}

@inproceedings{wan-2008-exploration-graph,
    title = "an exploration of document impact on graph-based multi-document summarization",
    author = "wan, xiaojun",
    booktitle = "proceedings of the 2008 conference on empirical methods in natural language processing",
    month = oct,
    year = "2008",
    address = "honolulu, hawaii",
    publisher = "association for computational linguistics",
    url = "https://www.aclweb.org/anthology/d08-1079",
    pages = "755--762",
}

@inproceedings{mmr,
 author = {carbonell, jaime and goldstein, jade},
 title = {the use of mmr, diversity-based reranking for reordering documents and producing summaries},
 booktitle = {proceedings of the 21st annual international acm sigir conference on research and development in information retrieval},
 series = {sigir '98},
 year = {1998},
 isbn = {1-58113-015-5},
 location = {melbourne, australia},
 pages = {335--336},
 numpages = {2},
 url = {http://doi.acm.org/10.1145/290941.291025},
 doi = {10.1145/290941.291025},
 acmid = {291025},
 publisher = {acm},
 address = {new york, ny, usa},
} 

@inproceedings{lin2010multi,
  title={multi-document summarization via budgeted maximization of submodular functions},
  author={lin, hui and bilmes, jeff},
  booktitle={human language technologies: the 2010 annual conference of the north american chapter of the association for computational linguistics},
  pages={912--920},
  year={2010}
}

@inproceedings{ft-bert-extractive,
    title = "text summarization with pretrained encoders",
    author = "liu, yang  and
      lapata, mirella",
    booktitle = "proceedings of the 2019 conference on empirical methods in natural language processing and the 9th international joint conference on natural language processing (emnlp-ijcnlp)",
    month = nov,
    year = "2019",
    address = "hong kong, china",
    publisher = "association for computational linguistics",
    url = "https://aclanthology.org/d19-1387",
    doi = "10.18653/v1/d19-1387",
    pages = "3730--3740",
}

@inproceedings{c14-1001,
  author =	"harper, mary",
  title = 	"learning from 26 languages: program management and science in the babel program",
  booktitle = 	"proceedings of coling 2014, the 25th international conference on computational linguistics: technical papers",
  year =    "2014",
  publisher =	"dublin city university and association for computational linguistics",
  pages =   "1",
  location =	"dublin, ireland",
  url =    "http://aclweb.org/anthology/c14-1001"
}

@article{baumel2018query,
  title={query focused abstractive summarization: incorporating query relevance, multi-document coverage, and summary length constraints into seq2seq models},
  author={baumel, tal and eyal, matan and elhadad, michael},
  journal= {computing research repository},
  volume={arxiv:1801.07704},
  url = {https://arxiv.org/abs/1801.07704},
  year={2018}
}

@inproceedings{feigenblat2017,
 author = {feigenblat, guy and roitman, haggai and boni, odellia and konopnicki, david},
 title = {unsupervised query-focused multi-document summarization using the cross entropy method},
 booktitle = {proceedings of the 40th international acm sigir conference on research and development in information retrieval},
 series = {sigir '17},
 year = {2017},
 isbn = {978-1-4503-5022-8},
 location = {shinjuku, tokyo, japan},
 pages = {961--964},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/3077136.3080690},
 doi = {10.1145/3077136.3080690},
 acmid = {3080690},
 publisher = {acm},
 address = {new york, ny, usa},
 keywords = {cross entropy method, multidocument summarization},
}

@article{wikiasp,
	author = {hiroaki hayashi and prashant budania and peng wang and chris ackerson and raj neervannan and graham neubig},
	title = {wikiasp: a dataset for multi-domain aspect-based summarization},
	journal = {transactions of the association for computational linguistics},
	volume = {9},
	number = {0},
	year = {2021},
	keywords = {},
	issn = {2307-387x},	pages = {211--225},	url = {https://transacl.org/ojs/index.php/tacl/article/view/2511}
}



@inproceedings{aquamuse,
  	address = {cham},
	author = {kulkarni, sayali and chammas, sheide and zhu, wan and sha, fei and ie, eugene},
	journal = {document analysis and recognition -- icdar 2021},
	editor = {llad{\'o}s, josep and lopresti, daniel and uchida, seiichi},
	isbn = {978-3-030-86331-9},
	pages = {84--98},
	publisher = {springer international publishing},
	title = {comsum and sibert: a dataset and neural model for query-based multi-document summarization},
	year = {2021}
}

@article{kwiatkowski-etal-2019-natural,
    title = "natural questions: a benchmark for question answering research",
    author = "kwiatkowski, tom  and
      palomaki, jennimaria  and
      redfield, olivia  and
      collins, michael  and
      parikh, ankur  and
      alberti, chris  and
      epstein, danielle  and
      polosukhin, illia  and
      devlin, jacob  and
      lee, kenton  and
      toutanova, kristina  and
      jones, llion  and
      kelcey, matthew  and
      chang, ming-wei  and
      dai, andrew m.  and
      uszkoreit, jakob  and
      le, quoc  and
      petrov, slav",
    journal = "transactions of the association for computational linguistics",
    volume = "7",
    month = mar,
    year = "2019",
    url = "https://aclanthology.org/q19-1026",
    doi = "10.1162/tacl_a_00276",
    pages = "452--466",
}


@inproceedings{
j.2018generating,
title={generating wikipedia by summarizing long sequences},
author={peter j. liu* and mohammad saleh* and etienne pot and ben goodrich and ryan sepassi and lukasz kaiser and noam shazeer},
booktitle={international conference on learning representations},
year={2018},
url={https://openreview.net/forum?id=hyg0vbwc-},
}

@inproceedings{wsl-dl,
    title = "{wsl}-{ds}: weakly supervised learning with distant supervision for query focused multi-document abstractive summarization",
    author = "laskar, md tahmid rahman  and
      hoque, enamul  and
      huang, jimmy xiangji",
    booktitle = "proceedings of the 28th international conference on computational linguistics",
    month = dec,
    year = "2020",
    address = "barcelona, spain (online)",
    publisher = "international committee on computational linguistics",
    url = "https://aclanthology.org/2020.coling-main.495",
    doi = "10.18653/v1/2020.coling-main.495",
    pages = "5647--5654",
}


@inproceedings{cnndaily,
	author = {hermann, karl moritz and kocisky, tomas and grefenstette, edward and espeholt, lasse and kay, will and suleyman, mustafa and blunsom, phil},
	booktitle = {advances in neural information processing systems},
	editor = {c. cortes and n. lawrence and d. lee and m. sugiyama and r. garnett},
	publisher = {curran associates, inc.},
	title = {teaching machines to read and comprehend},
	url = {https://proceedings.neurips.cc/paper/2015/file/afdec7005cc9f14302cd0474fd0f3c96-paper.pdf},
	volume = {28},
	year = {2015},
	bdsk-url-1 = {https://proceedings.neurips.cc/paper/2015/file/afdec7005cc9f14302cd0474fd0f3c96-paper.pdf}}

@inproceedings{xu-lapata-2020-coarse,
    title = "coarse-to-fine query focused multi-document summarization",
    author = "xu, yumo  and
      lapata, mirella",
    booktitle = "proceedings of the 2020 conference on empirical methods in natural language processing (emnlp)",
    month = nov,
    year = "2020",
    address = "online",
    publisher = "association for computational linguistics",
    url = "https://aclanthology.org/2020.emnlp-main.296",
}

@inproceedings{dual_ces,
author = {roitman, haggai and feigenblat, guy and cohen, doron and boni, odellia and konopnicki, david},
title = {unsupervised dual-cascade learning with pseudo-feedback distillation for query-focused extractive summarization},
year = {2020},
isbn = {9781450370233},
publisher = {association for computing machinery},
address = {new york, ny, usa},
url = {https://doi.org/10.1145/3366423.3380009},
doi = {10.1145/3366423.3380009},
booktitle = {proceedings of the web conference 2020},
pages = {2577–2584},
numpages = {8},
location = {taipei, taiwan},
series = {www '20}
}

@incollection{pytorch,
	author = {paszke, adam and gross, sam and massa, francisco and lerer, adam and bradbury, james and chanan, gregory and killeen, trevor and lin, zeming and gimelshein, natalia and antiga, luca and desmaison, alban and kopf, andreas and yang, edward and devito, zachary and raison, martin and tejani, alykhan and chilamkurthy, sasank and steiner, benoit and fang, lu and bai, junjie and chintala, soumith},
	booktitle = {advances in neural information processing systems 32},
	editor = {h. wallach and h. larochelle and a. beygelzimer and f. d\textquotesingle alch\'{e}-buc and e. fox and r. garnett},
	pages = {8024--8035},
	publisher = {curran associates, inc.},
	title = {pytorch: an imperative style, high-performance deep learning library},
	url = {http://papers.neurips.cc/paper/9015-pytorch-an-imperative-style-high-performance-deep-learning-library.pdf},
	year = {2019}}
	
	@inproceedings{wolf-etal-2020-transformers,
    title = "transformers: state-of-the-art natural language processing",
    author = "wolf, thomas  and
      debut, lysandre  and
      sanh, victor  and
      chaumond, julien  and
      delangue, clement  and
      moi, anthony  and
      cistac, pierric  and
      rault, tim  and
      louf, remi  and
      funtowicz, morgan  and
      davison, joe  and
      shleifer, sam  and
      von platen, patrick  and
      ma, clara  and
      jernite, yacine  and
      plu, julien  and
      xu, canwen  and
      le scao, teven  and
      gugger, sylvain  and
      drame, mariama  and
      lhoest, quentin  and
      rush, alexander",
    booktitle = "proceedings of the 2020 conference on empirical methods in natural language processing: system demonstrations",
    month = oct,
    year = "2020",
    address = "online",
    publisher = "association for computational linguistics",
    url = "https://aclanthology.org/2020.emnlp-demos.6",
    doi = "10.18653/v1/2020.emnlp-demos.6",
    pages = "38--45",
}

@inproceedings{zhu2018to,
	author = {michael h. zhu and suyog gupta},
	booktitle = {international conference on learning representations, workshop track proceedings},
	title = {to prune, or not to prune: exploring the efficacy of pruning for model compression},
	url = {https://openreview.net/forum?id=s1ln69at-},
	year = {2018}}
	
	@inproceedings{wang-etal-2017-gated,
    title = "gated self-matching networks for reading comprehension and question answering",
    author = "wang, wenhui  and
      yang, nan  and
      wei, furu  and
      chang, baobao  and
      zhou, ming",
    booktitle = "proceedings of the 55th annual meeting of the association for computational linguistics (volume 1: long papers)",
    month = jul,
    year = "2017",
    address = "vancouver, canada",
    publisher = "association for computational linguistics",
    url = "https://aclanthology.org/p17-1018",
    doi = "10.18653/v1/p17-1018",
    pages = "189--198",
}

@article{roberta,
	archiveprefix = {arxiv},
	author = {yinhan liu and myle ott and naman goyal and jingfei du and mandar joshi and danqi chen and omer levy and mike lewis and luke zettlemoyer and veselin stoyanov},
	eprint = {1907.11692},
	journal = {corr},
	title = {roberta: {a} robustly optimized {bert} pretraining approach},
	url = {http://arxiv.org/abs/1907.11692},
	volume = {abs/1907.11692},
	year = {2019}}
	
@inproceedings{xlnet,
	author = {zhilin yang and zihang dai and yiming yang and jaime g. carbonell and ruslan salakhutdinov and quoc v. le},
	booktitle = {advances in neural information processing systems 32: annual conference on neural information processing systems 2019, neurips 2019, december 8-14, 2019, vancouver, bc, canada},
	pages = {5754--5764},
	title = {xlnet: generalized autoregressive pretraining for language understanding},
	url = {https://proceedings.neurips.cc/paper/2019/hash/dc6a7e655d7e5840e66733e9ee67cc69-abstract.html},
	year = {2019}}
	
@inproceedings{unilm,
	author = {li dong and nan yang and wenhui wang and furu wei and xiaodong liu and yu wang and jianfeng gao and ming zhou and hsiao{-}wuen hon},
	booktitle = {advances in neural information processing systems 32: annual conference on neural information processing systems 2019, neurips 2019, december 8-14, 2019, vancouver, bc, canada},
	pages = {13042--13054},
	title = {unified language model pre-training for natural language understanding and generation},
	url = {https://proceedings.neurips.cc/paper/2019/hash/c20bb2d9a50d5ac1f713f8b34d9aac5a-abstract.html},
	year = {2019}}

@inproceedings{albert,
title={albert: a lite bert for self-supervised learning of language representations},
author={zhenzhong lan and mingda chen and sebastian goodman and kevin gimpel and piyush sharma and radu soricut},
booktitle={international conference on learning representations},
year={2020},
url={https://openreview.net/forum?id=h1ea7aetvs}
}

@inproceedings{electra,
    title = "pre-training transformers as energy-based cloze models",
    author = "clark, kevin  and
      luong, minh-thang  and
      le, quoc  and
      manning, christopher d.",
    booktitle = "proceedings of the 2020 conference on empirical methods in natural language processing (emnlp)",
    month = nov,
    year = "2020",
    address = "online",
    publisher = "association for computational linguistics",
    url = "https://aclanthology.org/2020.emnlp-main.20",
    doi = "10.18653/v1/2020.emnlp-main.20",
    pages = "285--294",
}

@inproceedings{dblp:conf/emnlp/prasannarr20,
	author = {sai prasanna and anna rogers and anna rumshisky},
	booktitle = {proceedings of the 2020 conference on empirical methods in natural language processing, {emnlp} 2020, online, november 16-20, 2020},
	doi = {10.18653/v1/2020.emnlp-main.259},
	pages = {3208--3229},
	publisher = {association for computational linguistics},
	title = {when {bert} plays the lottery, all tickets are winning},
	url = {https://doi.org/10.18653/v1/2020.emnlp-main.259},
	year = {2020}}
	
@inproceedings{lottery-for-bert,
	author = {tianlong chen and jonathan frankle and shiyu chang and sijia liu and yang zhang and zhangyang wang and michael carbin},
	booktitle = {advances in neural information processing systems 33: annual conference on neural information processing systems 2020, neurips 2020, december 6-12, 2020, virtual},
	title = {the lottery ticket hypothesis for pre-trained {bert} networks},
	url = {https://proceedings.neurips.cc/paper/2020/hash/b6af2c9703f203a2794be03d443af2e3-abstract.html},
	year = {2020}}

@article{liang2021super,
  title={super tickets in pre-trained language models: from model compression to improving generalization},
  author={liang, chen and zuo, simiao and chen, minshuo and jiang, haoming and liu, xiaodong and he, pengcheng and zhao, tuo and chen, weizhu},
  journal={arxiv preprint arxiv:2105.12002},
  year={2021}
}
{"mode":"full","isactive":false}26 languages: program management and science in the babel program",
  booktitle = 	"proceedings of coling 2014, the 25th international conference on computational linguistics: technical papers",
  year =    "2014",
  publisher =	"dublin city university and association for computational linguistics",
  pages =   "1",
  location =	"dublin, ireland",
  url =    "http://aclweb.org/anthology/c14-1001"
}

@article{baumel2018query,
  title={query focused abstractive summarization: incorporating query relevance, multi-document coverage, and summary length constraints into seq2seq models},
  author={baumel, tal and eyal, matan and elhadad, michael},
  journal= {computing research repository},
  volume={arxiv:1801.07704},
  url = {https://arxiv.org/abs/1801.07704},
  year={2018}
}

@inproceedings{feigenblat2017,
 author = {feigenblat, guy and roitman, haggai and boni, odellia and konopnicki, david},
 title = {unsupervised query-focused multi-document summarization using the cross entropy method},
 booktitle = {proceedings of the 40th international acm sigir conference on research and development in information retrieval},
 series = {sigir '17},
 year = {2017},
 isbn = {978-1-4503-5022-8},
 location = {shinjuku, tokyo, japan},
 pages = {961--964},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/3077136.3080690},
 doi = {10.1145/3077136.3080690},
 acmid = {3080690},
 publisher = {acm},
 address = {new york, ny, usa},
 keywords = {cross entropy method, multidocument summarization},
}

@article{wikiasp,
	author = {hiroaki hayashi and prashant budania and peng wang and chris ackerson and raj neervannan and graham neubig},
	title = {wikiasp: a dataset for multi-domain aspect-based summarization},
	journal = {transactions of the association for computational linguistics},
	volume = {9},
	number = {0},
	year = {2021},
	keywords = {},
	issn = {2307-387x},	pages = {211--225},	url = {https://transacl.org/ojs/index.php/tacl/article/view/2511}
}



@article{kwiatkowski-etal-2019-natural,
    title = "natural questions: a benchmark for question answering research",
    author = "kwiatkowski, tom  and
      palomaki, jennimaria  and
      redfield, olivia  and
      collins, michael  and
      parikh, ankur  and
      alberti, chris  and
      epstein, danielle  and
      polosukhin, illia  and
      devlin, jacob  and
      lee, kenton  and
      toutanova, kristina  and
      jones, llion  and
      kelcey, matthew  and
      chang, ming-wei  and
      dai, andrew m.  and
      uszkoreit, jakob  and
      le, quoc  and
      petrov, slav",
    journal = "transactions of the association for computational linguistics",
    volume = "7",
    month = mar,
    year = "2019",
    url = "https://aclanthology.org/q19-1026",
    doi = "10.1162/tacl_a_00276",
    pages = "452--466",
}


@inproceedings{
j.2018generating,
title={generating wikipedia by summarizing long sequences},
author={peter j. liu* and mohammad saleh* and etienne pot and ben goodrich and ryan sepassi and lukasz kaiser and noam shazeer},
booktitle={international conference on learning representations},
year={2018},
url={https://openreview.net/forum?id=hyg0vbwc-},
}

@inproceedings{wsl-dl,
    title = "{wsl}-{ds}: weakly supervised learning with distant supervision for query focused multi-document abstractive summarization",
    author = "laskar, md tahmid rahman  and
      hoque, enamul  and
      huang, jimmy xiangji",
    booktitle = "proceedings of the 28th international conference on computational linguistics",
    month = dec,
    year = "2020",
    address = "barcelona, spain (online)",
    publisher = "international committee on computational linguistics",
    url = "https://aclanthology.org/2020.coling-main.495",
    doi = "10.18653/v1/2020.coling-main.495",
    pages = "5647--5654",
}


@inproceedings{cnndaily,
	author = {hermann, karl moritz and kocisky, tomas and grefenstette, edward and espeholt, lasse and kay, will and suleyman, mustafa and blunsom, phil},
	booktitle = {advances in neural information processing systems},
	editor = {c. cortes and n. lawrence and d. lee and m. sugiyama and r. garnett},
	publisher = {curran associates, inc.},
	title = {teaching machines to read and comprehend},
	url = {https://proceedings.neurips.cc/paper/2015/file/afdec7005cc9f14302cd0474fd0f3c96-paper.pdf},
	volume = {28},
	year = {2015},
	bdsk-url-1 = {https://proceedings.neurips.cc/paper/2015/file/afdec7005cc9f14302cd0474fd0f3c96-paper.pdf}}

@inproceedings{xu-lapata-2020-coarse,
    title = "coarse-to-fine query focused multi-document summarization",
    author = "xu, yumo  and
      lapata, mirella",
    booktitle = "proceedings of the 2020 conference on empirical methods in natural language processing (emnlp)",
    month = nov,
    year = "2020",
    address = "online",
    publisher = "association for computational linguistics",
    url = "https://aclanthology.org/2020.emnlp-main.296",
}

@inproceedings{dual_ces,
author = {roitman, haggai and feigenblat, guy and cohen, doron and boni, odellia and konopnicki, david},
title = {unsupervised dual-cascade learning with pseudo-feedback distillation for query-focused extractive summarization},
year = {2020},
isbn = {9781450370233},
publisher = {association for computing machinery},
address = {new york, ny, usa},
url = {https://doi.org/10.1145/3366423.3380009},
doi = {10.1145/3366423.3380009},
booktitle = {proceedings of the web conference 2020},
pages = {2577–2584},
numpages = {8},
location = {taipei, taiwan},
series = {www '20}
}

@incollection{pytorch,
	author = {paszke, adam and gross, sam and massa, francisco and lerer, adam and bradbury, james and chanan, gregory and killeen, trevor and lin, zeming and gimelshein, natalia and antiga, luca and desmaison, alban and kopf, andreas and yang, edward and devito, zachary and raison, martin and tejani, alykhan and chilamkurthy, sasank and steiner, benoit and fang, lu and bai, junjie and chintala, soumith},
	booktitle = {advances in neural information processing systems 32},
	editor = {h. wallach and h. larochelle and a. beygelzimer and f. d\textquotesingle alch\'{e}-buc and e. fox and r. garnett},
	pages = {8024--8035},
	publisher = {curran associates, inc.},
	title = {pytorch: an imperative style, high-performance deep learning library},
	url = {http://papers.neurips.cc/paper/9015-pytorch-an-imperative-style-high-performance-deep-learning-library.pdf},
	year = {2019}}
	
	@inproceedings{wolf-etal-2020-transformers,
    title = "transformers: state-of-the-art natural language processing",
    author = "wolf, thomas  and
      debut, lysandre  and
      sanh, victor  and
      chaumond, julien  and
      delangue, clement  and
      moi, anthony  and
      cistac, pierric  and
      rault, tim  and
      louf, remi  and
      funtowicz, morgan  and
      davison, joe  and
      shleifer, sam  and
      von platen, patrick  and
      ma, clara  and
      jernite, yacine  and
      plu, julien  and
      xu, canwen  and
      le scao, teven  and
      gugger, sylvain  and
      drame, mariama  and
      lhoest, quentin  and
      rush, alexander",
    booktitle = "proceedings of the 2020 conference on empirical methods in natural language processing: system demonstrations",
    month = oct,
    year = "2020",
    address = "online",
    publisher = "association for computational linguistics",
    url = "https://aclanthology.org/2020.emnlp-demos.6",
    doi = "10.18653/v1/2020.emnlp-demos.6",
    pages = "38--45",
}

@inproceedings{zhu2018to,
	author = {michael h. zhu and suyog gupta},
	booktitle = {international conference on learning representations, workshop track proceedings},
	title = {to prune, or not to prune: exploring the efficacy of pruning for model compression},
	url = {https://openreview.net/forum?id=s1ln69at-},
	year = {2018}}
	
	@inproceedings{wang-etal-2017-gated,
    title = "gated self-matching networks for reading comprehension and question answering",
    author = "wang, wenhui  and
      yang, nan  and
      wei, furu  and
      chang, baobao  and
      zhou, ming",
    booktitle = "proceedings of the 55th annual meeting of the association for computational linguistics (volume 1: long papers)",
    month = jul,
    year = "2017",
    address = "vancouver, canada",
    publisher = "association for computational linguistics",
    url = "https://aclanthology.org/p17-1018",
    doi = "10.18653/v1/p17-1018",
    pages = "189--198",
}

@article{roberta,
	archiveprefix = {arxiv},
	author = {yinhan liu and myle ott and naman goyal and jingfei du and mandar joshi and danqi chen and omer levy and mike lewis and luke zettlemoyer and veselin stoyanov},
	eprint = {1907.11692},
	journal = {corr},
	title = {roberta: {a} robustly optimized {bert} pretraining approach},
	url = {http://arxiv.org/abs/1907.11692},
	volume = {abs/1907.11692},
	year = {2019}}
	
@inproceedings{xlnet,
	author = {zhilin yang and zihang dai and yiming yang and jaime g. carbonell and ruslan salakhutdinov and quoc v. le},
	booktitle = {advances in neural information processing systems 32: annual conference on neural information processing systems 2019, neurips 2019, december 8-14, 2019, vancouver, bc, canada},
	pages = {5754--5764},
	title = {xlnet: generalized autoregressive pretraining for language understanding},
	url = {https://proceedings.neurips.cc/paper/2019/hash/dc6a7e655d7e5840e66733e9ee67cc69-abstract.html},
	year = {2019}}
	
@inproceedings{unilm,
	author = {li dong and nan yang and wenhui wang and furu wei and xiaodong liu and yu wang and jianfeng gao and ming zhou and hsiao{-}wuen hon},
	booktitle = {advances in neural information processing systems 32: annual conference on neural information processing systems 2019, neurips 2019, december 8-14, 2019, vancouver, bc, canada},
	pages = {13042--13054},
	title = {unified language model pre-training for natural language understanding and generation},
	url = {https://proceedings.neurips.cc/paper/2019/hash/c20bb2d9a50d5ac1f713f8b34d9aac5a-abstract.html},
	year = {2019}}

@inproceedings{albert,
title={albert: a lite bert for self-supervised learning of language representations},
author={zhenzhong lan and mingda chen and sebastian goodman and kevin gimpel and piyush sharma and radu soricut},
booktitle={international conference on learning representations},
year={2020},
url={https://openreview.net/forum?id=h1ea7aetvs}
}

@inproceedings{electra,
    title = "pre-training transformers as energy-based cloze models",
    author = "clark, kevin  and
      luong, minh-thang  and
      le, quoc  and
      manning, christopher d.",
    booktitle = "proceedings of the 2020 conference on empirical methods in natural language processing (emnlp)",
    month = nov,
    year = "2020",
    address = "online",
    publisher = "association for computational linguistics",
    url = "https://aclanthology.org/2020.emnlp-main.20",
    doi = "10.18653/v1/2020.emnlp-main.20",
    pages = "285--294",
}

@inproceedings{dblp:conf/emnlp/prasannarr20,
	author = {sai prasanna and anna rogers and anna rumshisky},
	booktitle = {proceedings of the 2020 conference on empirical methods in natural language processing, {emnlp} 2020, online, november 16-20, 2020},
	doi = {10.18653/v1/2020.emnlp-main.259},
	pages = {3208--3229},
	publisher = {association for computational linguistics},
	title = {when {bert} plays the lottery, all tickets are winning},
	url = {https://doi.org/10.18653/v1/2020.emnlp-main.259},
	year = {2020}}
	
@inproceedings{lottery-for-bert,
	author = {tianlong chen and jonathan frankle and shiyu chang and sijia liu and yang zhang and zhangyang wang and michael carbin},
	booktitle = {advances in neural information processing systems 33: annual conference on neural information processing systems 2020, neurips 2020, december 6-12, 2020, virtual},
	title = {the lottery ticket hypothesis for pre-trained {bert} networks},
	url = {https://proceedings.neurips.cc/paper/2020/hash/b6af2c9703f203a2794be03d443af2e3-abstract.html},
	year = {2020}}

@article{liang2021super,
  title={super tickets in pre-trained language models: from model compression to improving generalization},
  author={liang, chen and zuo, simiao and chen, minshuo and jiang, haoming and liu, xiaodong and he, pengcheng and zhao, tuo and chen, weizhu},
  journal={arxiv preprint arxiv:2105.12002},
  year={2021}
}

@inproceedings{hibert,
    title = "{hibert}: document level pre-training of hierarchical bidirectional transformers for document summarization",
    author = "zhang, xingxing  and
      wei, furu  and
      zhou, ming",
    booktitle = "proceedings of the 57th annual meeting of the association for computational linguistics",
    month = jul,
    year = "2019",
    address = "florence, italy",
    publisher = "association for computational linguistics",
    url = "https://aclanthology.org/p19-1499",
    doi = "10.18653/v1/p19-1499",
    pages = "5059--5069",
}


@inproceedings{aquamuse,
author="kulkarni, sayali
and chammas, sheide
and zhu, wan
and sha, fei
and ie, eugene",
editor="llad{\'o}s, josep
and lopresti, daniel
and uchida, seiichi",
title="comsum and sibert: a dataset and neural model for query-based multi-document summarization",
booktitle="document analysis and recognition -- icdar 2021",
year="2021",
publisher="springer international publishing",
address="cham",
pages="84--98",
isbn="978-3-030-86331-9"
}


